Recurrent Memory Networks for Language Modeling

Recurrent Neural Networks (RNN) have obtained excellent result in many natural language processing (NLP) tasks. However, understanding and interpreting the source of this success remains a challenge. In this paper, we propose Recurrent Memory Network (RMN), a novel RNN architecture, that not only amplifies the power of RNN but also facilitates our understanding of its internal functioning and allows us to discover underlying patterns in data. We demonstrate the power of RMN on language modeling and sentence completion tasks. On language modeling, RMN outperforms Long Short-Term Memory (LSTM) network on three large German, Italian, and English dataset. Additionally we perform in-depth analysis of various linguistic dimensions that RMN captures. On Sentence Completion Challenge, for which it is essential to capture sentence coherence, our RMN obtains 69.2% accuracy, surpassing the previous state-of-the-art by a large margin.

==> table-attend-examples.tex <==
\begin{figure*}[t]
\centering
   \begin{subfigure}[b]{0.93\textwidth}
   \includegraphics[width=1\linewidth]{figs/de_sv.pdf}
   \caption{Separable verb. Gloss: \textit{effective the from-that resulting strategy will be , depends therefore on the accuracy these measures}}
   \label{fig:example_sv} 
\end{subfigure}
\begin{subfigure}[b]{0.93\textwidth}
   \includegraphics[width=1\linewidth]{figs/de_fex.pdf}
   \caption{Fixed expression. Gloss: \textit{the position place willl, a key-role in the restriction of-the regional ambitions China's to}}
   \phantomsubcaption\label{fig:example_fe}
\end{subfigure}
\caption{Examples of attention distribution over memory positions when predicting the next word. \AB{The predicted word must also be in the figure! (but marked differently). English translation (not just gloss) should also be there.}}
\end{figure*}
